Beyond One-Hot-Encoding: Injecting Semantics to Drive Image Classifiers

Images are loaded with semantic information that pertains to real-world ontologies: dog breeds share mammalian similarities, food pictures are often depicted in domestic environments, and so on. However, when training machine learning models for image classification, the relative similarities amongst object classes are commonly paired with one-hot-encoded labels. According to this logic, if an image is labelled as 'spoon', then 'tea-spoon' and 'shark' are equally wrong in terms of training loss. To overcome this limitation, we explore the integration of additional goals that reflect ontological and semantic knowledge, improving model interpretability and trustworthiness. We suggest a generic approach that allows to derive an additional loss term starting from any kind of semantic information about the classification label. First, we show how to apply our approach to ontologies and word embeddings, and discuss how the resulting information can drive a supervised learning process. Second, we use our semantically enriched loss to train image classifiers, and analyse the trade-offs between accuracy, mistake severity, and learned internal representations. Finally, we discuss how this approach can be further exploited in terms of explainability and adversarial robustness. Code repository: https://github.com/S1M0N38/semantic-encodings

==> _tables/4A.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
level & \multicolumn{10}{l}{0} \\
scores (↓) & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{avg\_hier\_dist\_k\_1} & \multicolumn{2}{l}{avg\_hier\_dist\_k\_5} & \multicolumn{2}{l}{avg\_hier\_dist\_k\_20} \\
{} &   mean &   std &              mean &   std &              mean &   std &              mean &   std &               mean &   std \\
\midrule
xent\_v3\_100            & 22.462 & 0.283 &             2.364 & 0.025 &             0.531 & 0.004 &             2.242 & 0.006 &              3.178 & 0.008 \\
haf\_v3\_100             & 22.327 & 0.078 &             2.246 & 0.023 &             0.501 & 0.003 &             1.417 & 0.008 &              2.640 & 0.001 \\
emb\_v3\_b0.40\_100       & 22.718 & 0.267 &             2.218 & 0.021 &             0.504 & 0.004 &             1.233 & 0.004 &              2.192 & 0.002 \\
emb\_v3\_b0.70\_100\_glove & 22.206 & 0.430 &             2.307 & 0.022 &             0.512 & 0.013 &             1.914 & 0.005 &              2.843 & 0.002 \\
\bottomrule
\end{tabular}


==> _tables/4A_COMPLETE.tex <==
\begin{table}[h]
\begin{tabularx}{\textwidth}{l|XXXXX}
\toprule
$(\downarrow)$ & Error  & MS  & HD@1 & HD@5  & HD@20  \\
\hline
XENT  \hspace*{2cm}             &                     22.462 &                    2.364 &                                  0.531 &              2.242&               3.178\\
SOFT-4   &                     32.580 &                            2.206 &                      0.719 &                      1.235 &                       2.223 \\
SOFT-30  &                     26.650 &                            2.331 &                      0.621 &                      1.375 &                       2.798 \\
HAF        &             22.420         &                    2.251         &              0.505  &              1.422  &               2.640  \\
HT-AL $(\beta = 0.30)$ &                     23.390 &                            2.237 &                      0.523 &                      1.233 &                       2.195 \\
HT-AL $(\beta = 0.35)$ &                     22.820 &                            2.252 &                      0.514 &                      1.236 &                       2.195 \\
HT-AL $(\beta = 0.40)$ &             22.718  &                    2.218  &              0.504  &              1.233  &               2.192  \\
HT-AL $(\beta = 0.45)$ &                     22.760 &                            2.219 &                      0.505 &                      1.242 &                       2.194 \\
HT-AL $(\beta = 0.50)$ &                     22.710 &                            2.262 &                      0.514 &                      1.256 &                       2.199 \\
WE-AL $(\beta = 0.30)$ &                     23.230 &                            2.303 &                      0.535 &                      1.836 &                       2.808 \\
WE-AL $(\beta = 0.35)$ &                     23.270 &                            2.312 &                      0.538 &                      1.841 &                       2.817 \\
WE-AL $(\beta = 0.40)$ &                     23.260 &                            2.311 &                      0.538 &                      1.851 &                       2.822 \\
WE-AL $(\beta = 0.45)$ &                     22.870 &                            2.320 &                      0.530 &                      1.849 &                       2.815 \\
WE-AL $(\beta = 0.50)$ &                     22.760 &                            2.291 &                      0.521 &                      1.864 &                       2.823 \\
WE-AL $(\beta = 0.55)$ &                     22.380 &                            2.332 &                      0.522 &                      1.879 &                       2.824 \\
WE-AL $(\beta = 0.60)$ &                     22.490 &                            2.349 &                      0.528 &                      1.887 &                       2.833 \\
WE-AL $(\beta = 0.65)$ &                     22.450 &                            2.325 &                      0.522 &                      1.907 &                       2.834 \\
WE-AL $(\beta = 0.70)$ &             22.206  &                    2.307  &              0.512  &              1.914  &               2.843  \\
WE-AL $(\beta = 0.75)$ &                     22.270 &                            2.302 &                      0.513 &                      1.931 &                       2.853 \\
\bottomrule
\end{tabularx}
\vspace*{2mm}
\caption{Accuracy and mistake severity for all trained ML models.}
\label{tab:ml_all}
%\end{center}
\end{table}

==> _tables/4A_T_COMPLETE.tex <==
\begin{tabular}{llllllllllllllllllll}
\toprule
{} &   Cross Entropy & Soft Labels $(\beta = 4)$ & Soft Labels $(\beta = 30)$ & Hier. Aware Features & Hier. Emb. $(\beta = 0.30)$ & Hier. Emb. $(\beta = 0.35)$ & Hier. Emb. $(\beta = 0.40)$ & Hier. Emb. $(\beta = 0.45)$ & Hier. Emb. $(\beta = 0.50)$ & GloVe Emb. $(\beta = 0.30)$ & GloVe Emb. $(\beta = 0.35)$ & GloVe Emb. $(\beta = 0.40)$ & GloVe Emb. $(\beta = 0.45)$ & GloVe Emb. $(\beta = 0.50)$ & GloVe Emb. $(\beta = 0.55)$ & GloVe Emb. $(\beta = 0.60)$ & GloVe Emb. $(\beta = 0.65)$ & GloVe Emb. $(\beta = 0.70)$ & GloVe Emb. $(\beta = 0.75)$ \\
\midrule
Top-1 Error $(\downarrow)$       &  22.462 ± 0.283 &                    32.580 &                     26.650 &       22.420 ± 0.203 &                      23.390 &                      22.820 &              22.718 ± 0.267 &                      22.760 &                      22.710 &                      23.230 &                      23.270 &                      23.260 &                      22.870 &                      22.760 &                      22.380 &                      22.490 &                      22.450 &              22.206 ± 0.430 &                      22.270 \\
Mistakes severity $(\downarrow)$ &   2.364 ± 0.025 &                     2.206 &                      2.331 &        2.251 ± 0.018 &                       2.237 &                       2.252 &               2.218 ± 0.021 &                       2.219 &                       2.262 &                       2.303 &                       2.312 &                       2.311 &                       2.320 &                       2.291 &                       2.332 &                       2.349 &                       2.325 &               2.307 ± 0.022 &                       2.302 \\
Hier dist@1 $(\downarrow)$       &   0.531 ± 0.004 &                     0.719 &                      0.621 &        0.505 ± 0.005 &                       0.523 &                       0.514 &               0.504 ± 0.004 &                       0.505 &                       0.514 &                       0.535 &                       0.538 &                       0.538 &                       0.530 &                       0.521 &                       0.522 &                       0.528 &                       0.522 &               0.512 ± 0.013 &                       0.513 \\
Hier dist@5 $(\downarrow)$       &   2.242 ± 0.006 &                     1.235 &                      1.375 &        1.422 ± 0.011 &                       1.233 &                       1.236 &               1.233 ± 0.004 &                       1.242 &                       1.256 &                       1.836 &                       1.841 &                       1.851 &                       1.849 &                       1.864 &                       1.879 &                       1.887 &                       1.907 &               1.914 ± 0.005 &                       1.931 \\
Hier dist@20 $(\downarrow)$      &   3.178 ± 0.008 &                     2.223 &                      2.798 &        2.640 ± 0.005 &                       2.195 &                       2.195 &               2.192 ± 0.002 &                       2.194 &                       2.199 &                       2.808 &                       2.817 &                       2.822 &                       2.815 &                       2.823 &                       2.824 &                       2.833 &                       2.834 &               2.843 ± 0.002 &                       2.853 \\
\bottomrule
\end{tabular}


==> _tables/4A_v2.tex <==
\begin{table}[h]
\begin{center}
\begin{tabularx}{\textwidth}{|l|X|X|X|X|X|}
\hline
{} & \textbf{XENT} & \textbf{HAF} & \textbf{SALT-HIER ($\beta$0.4)} & \textbf{SALT-WEMB ($\beta$0.7)} & X\\
\hline
%0 &    xent\_v3\_100 &     haf\_v3\_100 &  emb\_v3\_b0.40\_100 &  emb\_v3\_b0.70\_100\_glove \\
error &  22.462$\pm$0.283 &  22.327$\pm$0.078 &     22.718$\pm$0.267 &           22.206$\pm$0.430 & X\\
\hline
hier\_dist\_mistake &   2.364$\pm$0.025 &   2.246$\pm$0.023 &      2.218$\pm$0.021 &            2.307$\pm$0.022 & X\\
\hline
avg\_hier\_dist\_k\_1 &   0.531$\pm$0.004 &   0.501$\pm$0.003 &      0.504$\pm$0.004 &            0.512$\pm$0.013 & X\\
\hline
avg\_hier\_dist\_k\_5 &   2.242$\pm$0.006 &   1.417$\pm$0.008 &      1.233$\pm$0.004 &            1.914$\pm$0.005 & X\\
\hline
avg\_hier\_dist\_k\_20 &   3.178$\pm$0.008 &   2.640$\pm$0.001 &      2.192$\pm$0.002 &            2.843$\pm$0.002 & X\\
\hline
\end{tabularx}
\vspace*{2mm}
\caption{Accuracy and mistake severity for our selected models}
\label{tab:models}
\end{center}
\end{table}

==> _tables/4A_v3.tex <==
\begin{table}[h]
%\begin{center}
%\hspace{-1cm}
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\textbf{(↓)} & error & \textit{HDM} & \textit{HD-k1} & \textit{HD-k5} & \textit{HD-k20}\\
\hline
XENT &  22.462$\pm$0.283 &  2.364$\pm$0.025 &  0.531$\pm$0.004 &  2.242$\pm$0.006 &  3.178$\pm$0.008 \\
\hline
SOFT4 &  ? &  ? &  ? &  ? &  ? \\
\hline
SOFT30 &  ? &  ? &  ? &  ? &  ? \\
\hline
HAF &  22.327$\pm$0.078 &  2.246$\pm$0.023 &  0.501$\pm$0.003 &  1.417$\pm$0.008 &  2.640$\pm$0.001 \\
\hline
HT-AL.4 &  22.718$\pm$0.267 &  2.218$\pm$0.021 &  0.504$\pm$0.004 &  1.233$\pm$0.004 &  2.192$\pm$0.002 \\
\hline
HT-ALx &  ? &  ? &  ? &  ? &  ? \\
\hline
WE-AL.7 &  22.206$\pm$0.430 &  2.307$\pm$0.022 &  0.512$\pm$0.013 &  1.914$\pm$0.005 &  2.843$\pm$0.002 \\
\hline
WE-ALx &  ? &  ? &  ? &  ? &  ? \\
\hline
\end{tabular}
%\vspace*{2mm}
\caption{Accuracy and mistake severity for all trained ML models. QQQ}
\label{tab:ml_all}
%\end{center}
\end{table}

==> _tables/4B.tex <==
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
\toprule
level & \multicolumn{4}{l}{0} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{2} & \multicolumn{4}{l}{3} & \multicolumn{4}{l}{4} \\
scores (↓) & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} \\
{} &   mean &   std &              mean &   std &   mean &   std &              mean &   std &  mean &   std &              mean &   std &  mean &   std &              mean &   std &  mean &   std &              mean &   std \\
\midrule
xent\_v3\_100            & 22.462 & 0.283 &             2.364 & 0.025 & 14.002 & 0.170 &             2.188 & 0.027 & 9.182 & 0.184 &             1.812 & 0.026 & 4.488 & 0.108 &             1.661 & 0.020 & 2.966 & 0.131 &             1.000 & 0.000 \\
haf\_v3\_100             & 22.327 & 0.078 &             2.246 & 0.023 & 13.353 & 0.061 &             2.083 & 0.040 & 8.320 & 0.096 &             1.739 & 0.041 & 3.720 & 0.140 &             1.651 & 0.043 & 2.427 & 0.250 &             1.000 & 0.000 \\
emb\_v3\_b0.40\_100       & 22.718 & 0.267 &             2.218 & 0.021 & 13.554 & 0.153 &             2.042 & 0.023 & 8.312 & 0.128 &             1.698 & 0.020 & 3.552 & 0.119 &             1.635 & 0.018 & 2.254 & 0.094 &             1.000 & 0.000 \\
emb\_v3\_b0.70\_100\_glove & 22.206 & 0.430 &             2.307 & 0.022 & 13.598 & 0.396 &             2.134 & 0.027 & 8.652 & 0.283 &             1.782 & 0.013 & 4.088 & 0.167 &             1.656 & 0.012 & 2.682 & 0.144 &             1.000 & 0.000 \\
\bottomrule
\end{tabular}


==> _tables/4B_COMPLETE.tex <==
\begin{tabular}{lllllllllll}
\toprule
Level & \multicolumn{2}{l}{0} & \multicolumn{2}{l}{1} & \multicolumn{2}{l}{2} & \multicolumn{2}{l}{3} & \multicolumn{2}{l}{4} \\
{} & Top-1 Error $(\downarrow)$ & Mistakes severity $(\downarrow)$ & Top-1 Error $(\downarrow)$ & Mistakes severity $(\downarrow)$ & Top-1 Error $(\downarrow)$ & Mistakes severity $(\downarrow)$ & Top-1 Error $(\downarrow)$ & Mistakes severity $(\downarrow)$ & Top-1 Error $(\downarrow)$ & Mistakes severity $(\downarrow)$ \\
\midrule
Cross Entropy               &             22.462 ± 0.283 &                    2.364 ± 0.025 &             14.002 ± 0.170 &                    2.188 ± 0.027 &              9.182 ± 0.184 &                    1.812 ± 0.026 &              4.488 ± 0.108 &                    1.661 ± 0.020 &              2.966 ± 0.131 &                    1.000 ± 0.000 \\
Soft Labels $(\beta = 4)$   &                     32.580 &                            2.206 &                     19.630 &                            2.002 &                     11.320 &                            1.738 &                      4.970 &                            1.680 &                      3.380 &                            1.000 \\
Soft Labels $(\beta = 30)$  &                     26.650 &                            2.331 &                     16.690 &                            2.125 &                     10.420 &                            1.801 &                      5.020 &                            1.663 &                      3.330 &                            1.000 \\
Hier. Aware Features        &             22.420 ± 0.203 &                    2.251 ± 0.018 &             13.470 ± 0.188 &                    2.082 ± 0.029 &              8.372 ± 0.107 &                    1.741 ± 0.030 &              3.780 ± 0.129 &                    1.641 ± 0.034 &              2.424 ± 0.177 &                    1.000 ± 0.000 \\
Hier. Emb. $(\beta = 0.30)$ &                     23.390 &                            2.237 &                     14.070 &                            2.056 &                      8.640 &                            1.720 &                      3.740 &                            1.663 &                      2.480 &                            1.000 \\
Hier. Emb. $(\beta = 0.35)$ &                     22.820 &                            2.252 &                     13.920 &                            2.052 &                      8.640 &                            1.694 &                      3.710 &                            1.617 &                      2.290 &                            1.000 \\
Hier. Emb. $(\beta = 0.40)$ &             22.718 ± 0.267 &                    2.218 ± 0.021 &             13.554 ± 0.153 &                    2.042 ± 0.023 &              8.312 ± 0.128 &                    1.698 ± 0.020 &              3.552 ± 0.119 &                    1.635 ± 0.018 &              2.254 ± 0.094 &                    1.000 ± 0.000 \\
Hier. Emb. $(\beta = 0.45)$ &                     22.760 &                            2.219 &                     13.540 &                            2.049 &                      8.390 &                            1.694 &                      3.500 &                            1.663 &                      2.320 &                            1.000 \\
Hier. Emb. $(\beta = 0.50)$ &                     22.710 &                            2.262 &                     13.870 &                            2.066 &                      8.540 &                            1.732 &                      3.780 &                            1.653 &                      2.470 &                            1.000 \\
GloVe Emb. $(\beta = 0.30)$ &                     23.230 &                            2.303 &                     14.460 &                            2.093 &                      8.950 &                            1.765 &                      4.110 &                            1.667 &                      2.740 &                            1.000 \\
GloVe Emb. $(\beta = 0.35)$ &                     23.270 &                            2.312 &                     14.290 &                            2.137 &                      9.070 &                            1.792 &                      4.330 &                            1.658 &                      2.850 &                            1.000 \\
GloVe Emb. $(\beta = 0.40)$ &                     23.260 &                            2.311 &                     14.350 &                            2.125 &                      9.250 &                            1.746 &                      4.220 &                            1.635 &                      2.680 &                            1.000 \\
GloVe Emb. $(\beta = 0.45)$ &                     22.870 &                            2.320 &                     14.290 &                            2.112 &                      8.890 &                            1.787 &                      4.270 &                            1.639 &                      2.730 &                            1.000 \\
GloVe Emb. $(\beta = 0.50)$ &                     22.760 &                            2.291 &                     13.770 &                            2.134 &                      8.900 &                            1.755 &                      3.990 &                            1.684 &                      2.730 &                            1.000 \\
GloVe Emb. $(\beta = 0.55)$ &                     22.380 &                            2.332 &                     13.870 &                            2.150 &                      9.030 &                            1.766 &                      4.150 &                            1.667 &                      2.770 &                            1.000 \\
GloVe Emb. $(\beta = 0.60)$ &                     22.490 &                            2.349 &                     13.980 &                            2.171 &                      9.350 &                            1.751 &                      4.220 &                            1.664 &                      2.800 &                            1.000 \\
GloVe Emb. $(\beta = 0.65)$ &                     22.450 &                            2.325 &                     14.000 &                            2.124 &                      8.850 &                            1.779 &                      4.090 &                            1.685 &                      2.800 &                            1.000 \\
GloVe Emb. $(\beta = 0.70)$ &             22.206 ± 0.430 &                    2.307 ± 0.022 &             13.598 ± 0.396 &                    2.134 ± 0.027 &              8.652 ± 0.283 &                    1.782 ± 0.013 &              4.088 ± 0.167 &                    1.656 ± 0.012 &              2.682 ± 0.144 &                    1.000 ± 0.000 \\
GloVe Emb. $(\beta = 0.75)$ &                     22.270 &                            2.302 &                     13.590 &                            2.133 &                      8.610 &                            1.789 &                      4.060 &                            1.672 &                      2.730 &                            1.000 \\
\bottomrule
\end{tabular}


==> _tables/4B_T_COMPLETE.tex <==
\begin{table}
\begin{tabularx}{\textwidth}{llXXXX}
\toprule
  &    &   XENT & HAF & HT-AL & WE-AL \\
Level \hspace*{5mm} & {} &                 &                      &                             &                             \\
\hline
0 & Error \hspace*{5mm} &  22.462 ± 0.283 &       22.420 ± 0.203 &              22.718 ± 0.267 &              22.206 ± 0.430 \\
  & MS &   2.364 ± 0.025 &        2.251 ± 0.018 &               2.218 ± 0.021 &               2.307 ± 0.022 \\
\hline
1 & Error &  14.002 ± 0.170 &       13.470 ± 0.188 &              13.554 ± 0.153 &              13.598 ± 0.396 \\
  & MS &   2.188 ± 0.027 &        2.082 ± 0.029 &               2.042 ± 0.023 &               2.134 ± 0.027 \\
\hline
2 & Error &   9.182 ± 0.184 &        8.372 ± 0.107 &               8.312 ± 0.128 &               8.652 ± 0.283 \\
  & MS &   1.812 ± 0.026 &        1.741 ± 0.030 &               1.698 ± 0.020 &               1.782 ± 0.013 \\
\hline
3 & Error &   4.488 ± 0.108 &        3.780 ± 0.129 &               3.552 ± 0.119 &               4.088 ± 0.167 \\
  & MS &   1.661 ± 0.020 &        1.641 ± 0.034 &               1.635 ± 0.018 &               1.656 ± 0.012 \\
\hline
4 & Error &   2.966 ± 0.131 &        2.424 ± 0.177 &               2.254 ± 0.094 &               2.682 ± 0.144 \\
  & MS &   1.000 ± 0.000 &        1.000 ± 0.000 &               1.000 ± 0.000 &               1.000 ± 0.000 \\
\bottomrule
\end{tabularx}
\vspace*{2mm}
\caption{Error and MS, at all hierarchical depths, for our selected models.}
\label{tab:ml_sel}
%\end{center}
\end{table}



==> _tables/4B_v2.tex <==
\begin{table}[h]
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrr}
\toprule
level & \multicolumn{4}{l}{0} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{2} & \multicolumn{4}{l}{3} & \multicolumn{4}{l}{4} \\
scores (↓) & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} & \multicolumn{2}{l}{error} & \multicolumn{2}{l}{hier\_dist\_mistake} \\
{} &   mean &   std &              mean &   std &   mean &   std &              mean &   std &  mean &   std &              mean &   std &  mean &   std &              mean &   std &  mean &   std &              mean &   std \\
\midrule
xent\_v3\_100            & 22.462 & 0.283 &             2.364 & 0.025 & 14.002 & 0.170 &             2.188 & 0.027 & 9.182 & 0.184 &             1.812 & 0.026 & 4.488 & 0.108 &             1.661 & 0.020 & 2.966 & 0.131 &             1.000 & 0.000 \\
haf\_v3\_100             & 22.327 & 0.078 &             2.246 & 0.023 & 13.353 & 0.061 &             2.083 & 0.040 & 8.320 & 0.096 &             1.739 & 0.041 & 3.720 & 0.140 &             1.651 & 0.043 & 2.427 & 0.250 &             1.000 & 0.000 \\
emb\_v3\_b0.40\_100       & 22.718 & 0.267 &             2.218 & 0.021 & 13.554 & 0.153 &             2.042 & 0.023 & 8.312 & 0.128 &             1.698 & 0.020 & 3.552 & 0.119 &             1.635 & 0.018 & 2.254 & 0.094 &             1.000 & 0.000 \\
emb\_v3\_b0.70\_100\_glove & 22.206 & 0.430 &             2.307 & 0.022 & 13.598 & 0.396 &             2.134 & 0.027 & 8.652 & 0.283 &             1.782 & 0.013 & 4.088 & 0.167 &             1.656 & 0.012 & 2.682 & 0.144 &             1.000 & 0.000 \\
\bottomrule
\end{tabular}
%\vspace*{2mm}
\caption{QQQ SOMETHING for the selected models.}
\label{tab:ml_sel}
%\end{center}
\end{table}

==> _tables/7A.tex <==
\begin{table}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrrr}
\toprule
level & \multicolumn{8}{l}{0} & \multicolumn{8}{l}{1} & \multicolumn{8}{l}{2} & \multicolumn{8}{l}{3} & \multicolumn{8}{l}{4} \\
scores (↑) & \multicolumn{2}{l}{silhouette} & \multicolumn{2}{l}{calinski\_harabasz} & \multicolumn{2}{l}{-davies\_bouldin} & \multicolumn{2}{l}{-sdbw} & \multicolumn{2}{l}{silhouette} & \multicolumn{2}{l}{calinski\_harabasz} & \multicolumn{2}{l}{-davies\_bouldin} & \multicolumn{2}{l}{-sdbw} & \multicolumn{2}{l}{silhouette} & \multicolumn{2}{l}{calinski\_harabasz} & \multicolumn{2}{l}{-davies\_bouldin} & \multicolumn{2}{l}{-sdbw} & \multicolumn{2}{l}{silhouette} & \multicolumn{2}{l}{calinski\_harabasz} & \multicolumn{2}{l}{-davies\_bouldin} & \multicolumn{2}{l}{-sdbw} & \multicolumn{2}{l}{silhouette} & \multicolumn{2}{l}{calinski\_harabasz} & \multicolumn{2}{l}{-davies\_bouldin} & \multicolumn{2}{l}{-sdbw} \\
{} &       mean &   std &              mean &   std &            mean &   std &   mean &   std &       mean &   std &              mean &   std &            mean &   std &   mean &   std &       mean &   std &              mean &   std &            mean &   std &   mean &   std &       mean &   std &              mean &    std &            mean &   std &   mean &   std &       mean &   std &              mean &    std &            mean &   std &   mean &   std \\
\midrule
xent\_v3\_100            &      0.211 & 0.002 &           162.475 & 1.286 &          -1.675 & 0.014 & -0.613 & 0.001 &      0.083 & 0.001 &           178.061 & 1.680 &          -3.080 & 0.021 & -0.863 & 0.001 &      0.052 & 0.001 &           220.977 & 2.012 &          -3.585 & 0.029 & -0.918 & 0.001 &      0.043 & 0.001 &           253.902 &  4.173 &          -4.109 & 0.030 & -0.933 & 0.002 &      0.037 & 0.001 &           302.590 &  8.927 &          -5.404 & 0.078 & -0.989 & 0.001 \\
haf\_v3\_100             &      0.234 & 0.001 &           272.963 & 0.729 &          -1.600 & 0.002 & -0.511 & 0.000 &      0.164 & 0.001 &           554.229 & 3.102 &          -2.069 & 0.002 & -0.697 & 0.001 &      0.157 & 0.001 &           842.864 & 3.869 &          -1.999 & 0.005 & -0.763 & 0.001 &      0.146 & 0.002 &          1041.603 &  5.807 &          -2.028 & 0.009 & -0.802 & 0.002 &      0.136 & 0.002 &          1519.912 & 23.083 &          -2.400 & 0.017 & -0.917 & 0.001 \\
emb\_v3\_b0.40\_100       &      0.280 & 0.003 &           298.309 & 3.191 &          -1.544 & 0.019 & -0.493 & 0.002 &      0.110 & 0.000 &           583.928 & 3.720 &          -2.940 & 0.012 & -0.688 & 0.001 &      0.098 & 0.001 &          1200.146 & 7.394 &          -2.841 & 0.019 & -0.717 & 0.001 &      0.121 & 0.002 &          2239.803 & 11.338 &          -2.311 & 0.023 & -0.736 & 0.003 &      0.311 & 0.002 &          5111.578 & 38.524 &          -1.312 & 0.004 & -0.799 & 0.000 \\
emb\_v3\_b0.70\_100\_glove &      0.299 & 0.004 &           181.251 & 2.211 &          -1.461 & 0.018 & -0.588 & 0.002 &      0.100 & 0.001 &           185.382 & 0.876 &          -3.118 & 0.020 & -0.859 & 0.001 &      0.059 & 0.001 &           250.881 & 1.551 &          -3.676 & 0.013 & -0.906 & 0.001 &      0.050 & 0.002 &           327.581 &  4.539 &          -3.580 & 0.025 & -0.922 & 0.001 &      0.050 & 0.001 &           467.394 &  6.867 &          -4.399 & 0.033 & -0.975 & 0.001 \\
\bottomrule
\end{tabular}
\caption{QQQ. Cluster validation metrics.}
\label{table:clustering-quality-results}
\end{table}


==> _tables/7A_COMPLETE.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
Level & \multicolumn{4}{l}{0} & \multicolumn{4}{l}{1} & \multicolumn{4}{l}{2} & \multicolumn{4}{l}{3} & \multicolumn{4}{l}{4} \\
{} & Silhouette $()$ & Calinski-Harabasz $()$ & Davies-Bouldin $(\downarrow)$ & S-Dbw $(\downarrow)$ & Silhouette $()$ & Calinski-Harabasz $()$ & Davies-Bouldin $(\downarrow)$ & S-Dbw $(\downarrow)$ & Silhouette $()$ & Calinski-Harabasz $()$ & Davies-Bouldin $(\downarrow)$ & S-Dbw $(\downarrow)$ & Silhouette $()$ & Calinski-Harabasz $()$ & Davies-Bouldin $(\downarrow)$ & S-Dbw $(\downarrow)$ & Silhouette $()$ & Calinski-Harabasz $()$ & Davies-Bouldin $(\downarrow)$ & S-Dbw $(\downarrow)$ \\
\midrule
Cross Entropy               &   0.211 ± 0.002 &        162.475 ± 1.286 &                 1.675 ± 0.014 &        0.613 ± 0.001 &   0.083 ± 0.001 &        178.061 ± 1.680 &                 3.080 ± 0.021 &        0.863 ± 0.001 &   0.052 ± 0.001 &        220.977 ± 2.012 &                 3.585 ± 0.029 &        0.918 ± 0.001 &   0.043 ± 0.001 &        253.902 ± 4.173 &                 4.109 ± 0.030 &        0.933 ± 0.002 &   0.037 ± 0.001 &        302.590 ± 8.927 &                 5.404 ± 0.078 &        0.989 ± 0.001 \\
Soft Labels $(\beta = 4)$   &           0.005 &                174.191 &                         4.170 &                0.599 &           0.133 &                697.942 &                         2.482 &                0.653 &           0.150 &               1274.482 &                         2.089 &                0.707 &           0.185 &               1904.641 &                         1.719 &                0.737 &           0.243 &               3301.624 &                         1.628 &                0.861 \\
Soft Labels $(\beta = 30)$  &           0.034 &                 65.470 &                         3.792 &                0.776 &           0.059 &                202.328 &                         3.215 &                0.849 &           0.046 &                288.984 &                         3.313 &                0.899 &           0.040 &                344.038 &                         3.526 &                0.920 &           0.049 &                447.573 &                         4.470 &                0.982 \\
Hier. Aware Features        &   0.232 ± 0.002 &        271.400 ± 3.134 &                 1.607 ± 0.012 &        0.512 ± 0.002 &   0.163 ± 0.002 &        552.785 ± 4.442 &                 2.075 ± 0.012 &        0.698 ± 0.001 &   0.156 ± 0.001 &        841.832 ± 3.939 &                 2.002 ± 0.005 &        0.763 ± 0.001 &   0.146 ± 0.001 &       1040.067 ± 5.357 &                 2.031 ± 0.007 &        0.802 ± 0.002 &   0.136 ± 0.002 &      1519.240 ± 19.142 &                 2.401 ± 0.014 &        0.917 ± 0.000 \\
Hier. Emb. $(\beta = 0.30)$ &           0.259 &                314.511 &                         1.604 &                0.484 &           0.108 &                668.594 &                         2.923 &                0.663 &           0.103 &               1402.706 &                         2.747 &                0.695 &           0.136 &               2637.556 &                         2.196 &                0.719 &           0.340 &               6000.125 &                         1.208 &                0.779 \\
Hier. Emb. $(\beta = 0.35)$ &           0.269 &                304.505 &                         1.591 &                0.490 &           0.109 &                621.402 &                         2.933 &                0.676 &           0.099 &               1292.209 &                         2.802 &                0.704 &           0.127 &               2424.529 &                         2.250 &                0.723 &           0.325 &               5532.914 &                         1.258 &                0.787 \\
Hier. Emb. $(\beta = 0.40)$ &   0.280 ± 0.003 &        298.309 ± 3.191 &                 1.544 ± 0.019 &        0.493 ± 0.002 &   0.110 ± 0.000 &        583.928 ± 3.720 &                 2.940 ± 0.012 &        0.688 ± 0.001 &   0.098 ± 0.001 &       1200.146 ± 7.394 &                 2.841 ± 0.019 &        0.717 ± 0.001 &   0.121 ± 0.002 &      2239.803 ± 11.338 &                 2.311 ± 0.023 &        0.736 ± 0.003 &   0.311 ± 0.002 &      5111.578 ± 38.524 &                 1.312 ± 0.004 &        0.799 ± 0.000 \\
Hier. Emb. $(\beta = 0.45)$ &           0.279 &                285.759 &                         1.543 &                0.501 &           0.110 &                550.120 &                         2.949 &                0.698 &           0.093 &               1120.036 &                         2.902 &                0.727 &           0.117 &               2091.728 &                         2.344 &                0.743 &           0.297 &               4749.922 &                         1.362 &                0.808 \\
Hier. Emb. $(\beta = 0.50)$ &           0.283 &                275.136 &                         1.541 &                0.508 &           0.108 &                512.461 &                         2.987 &                0.711 &           0.094 &               1041.996 &                         2.936 &                0.739 &           0.112 &               1933.137 &                         2.401 &                0.755 &           0.283 &               4387.649 &                         1.417 &                0.818 \\
GloVe Emb. $(\beta = 0.30)$ &           0.327 &                215.149 &                         1.346 &                0.554 &           0.112 &                218.489 &                         2.952 &                0.840 &           0.069 &                299.843 &                         3.398 &                0.895 &           0.060 &                392.698 &                         3.281 &                0.913 &           0.061 &                562.900 &                         4.014 &                0.975 \\
GloVe Emb. $(\beta = 0.35)$ &           0.324 &                210.460 &                         1.362 &                0.558 &           0.111 &                212.168 &                         2.954 &                0.843 &           0.068 &                289.362 &                         3.456 &                0.897 &           0.056 &                376.534 &                         3.341 &                0.912 &           0.058 &                536.805 &                         4.111 &                0.976 \\
GloVe Emb. $(\beta = 0.40)$ &           0.316 &                201.922 &                         1.391 &                0.567 &           0.108 &                205.671 &                         2.987 &                0.847 &           0.066 &                281.319 &                         3.494 &                0.899 &           0.058 &                367.173 &                         3.384 &                0.917 &           0.056 &                513.389 &                         4.205 &                0.977 \\
GloVe Emb. $(\beta = 0.45)$ &           0.318 &                199.929 &                         1.416 &                0.567 &           0.106 &                201.386 &                         3.036 &                0.850 &           0.065 &                275.931 &                         3.526 &                0.901 &           0.055 &                360.711 &                         3.421 &                0.917 &           0.056 &                512.611 &                         4.205 &                0.975 \\
GloVe Emb. $(\beta = 0.50)$ &           0.320 &                199.455 &                         1.403 &                0.568 &           0.108 &                199.034 &                         3.031 &                0.851 &           0.065 &                269.542 &                         3.561 &                0.902 &           0.056 &                352.178 &                         3.453 &                0.921 &           0.054 &                495.790 &                         4.276 &                0.976 \\
GloVe Emb. $(\beta = 0.55)$ &           0.315 &                193.542 &                         1.413 &                0.575 &           0.104 &                193.487 &                         3.062 &                0.854 &           0.063 &                263.976 &                         3.608 &                0.904 &           0.054 &                346.277 &                         3.484 &                0.920 &           0.054 &                491.852 &                         4.295 &                0.977 \\
GloVe Emb. $(\beta = 0.60)$ &           0.311 &                189.560 &                         1.425 &                0.578 &           0.103 &                188.449 &                         3.085 &                0.857 &           0.060 &                254.195 &                         3.670 &                0.906 &           0.050 &                332.324 &                         3.550 &                0.921 &           0.051 &                474.829 &                         4.367 &                0.976 \\
GloVe Emb. $(\beta = 0.65)$ &           0.302 &                185.155 &                         1.448 &                0.584 &           0.099 &                185.115 &                         3.125 &                0.859 &           0.060 &                251.537 &                         3.647 &                0.909 &           0.052 &                328.974 &                         3.579 &                0.925 &           0.051 &                465.493 &                         4.413 &                0.977 \\
GloVe Emb. $(\beta = 0.70)$ &   0.299 ± 0.004 &        181.251 ± 2.211 &                 1.461 ± 0.018 &        0.588 ± 0.002 &   0.100 ± 0.001 &        185.382 ± 0.876 &                 3.118 ± 0.020 &        0.859 ± 0.001 &   0.059 ± 0.001 &        250.881 ± 1.551 &                 3.676 ± 0.013 &        0.906 ± 0.001 &   0.050 ± 0.002 &        327.581 ± 4.539 &                 3.580 ± 0.025 &        0.922 ± 0.001 &   0.050 ± 0.001 &        467.394 ± 6.867 &                 4.399 ± 0.033 &        0.975 ± 0.001 \\
GloVe Emb. $(\beta = 0.75)$ &           0.287 &                174.097 &                         1.511 &                0.596 &           0.097 &                182.043 &                         3.140 &                0.861 &           0.058 &                245.835 &                         3.704 &                0.910 &           0.052 &                323.135 &                         3.607 &                0.926 &           0.049 &                463.184 &                         4.419 &                0.975 \\
\bottomrule
\end{tabular}


==> _tables/7A_T_COMPLETE.tex <==
\begin{table}
\begin{tabularx}{\textwidth}{ll|l|l|l|l}
\toprule
  &  &  XENT \hspace*{12mm} & HAF \hspace*{15mm} & HT-AL \hspace*{12mm} & WE-AL \\
Level & and Metric &                &                      &                             &                             \\
\hline
0 & Silhouette $(\uparrow)$ &  0.211 ± 0.002 &        0.232 ± 0.002 &               0.280 ± 0.003 &               0.299 ± 0.004 \\
  & S-Dbw $(\downarrow)$ &  0.613 ± 0.001 &        0.512 ± 0.002 &               0.493 ± 0.002 &               0.588 ± 0.002 \\
1 & Silhouette $(\uparrow)$ &  0.083 ± 0.001 &        0.163 ± 0.002 &               0.110 ± 0.000 &               0.100 ± 0.001 \\
  & S-Dbw $(\downarrow)$ &  0.863 ± 0.001 &        0.698 ± 0.001 &               0.688 ± 0.001 &               0.859 ± 0.001 \\
2 & Silhouette $(\uparrow)$ &  0.052 ± 0.001 &        0.156 ± 0.001 &               0.098 ± 0.001 &               0.059 ± 0.001 \\
  & S-Dbw $(\downarrow)$ &  0.918 ± 0.001 &        0.763 ± 0.001 &               0.717 ± 0.001 &               0.906 ± 0.001 \\
3 & Silhouette $(\uparrow)$ &  0.043 ± 0.001 &        0.146 ± 0.001 &               0.121 ± 0.002 &               0.050 ± 0.002 \\
  & S-Dbw $(\downarrow)$ &  0.933 ± 0.002 &        0.802 ± 0.002 &               0.736 ± 0.003 &               0.922 ± 0.001 \\
4 & Silhouette $(\uparrow)$ &  0.037 ± 0.001 &        0.136 ± 0.002 &               0.311 ± 0.002 &               0.050 ± 0.001 \\
  & S-Dbw $(\downarrow)$ &  0.989 ± 0.001 &        0.917 ± 0.000 &               0.799 ± 0.000 &               0.975 ± 0.001 \\
\bottomrule
\end{tabularx}
\vspace*{2mm}
\caption{Clustering evaluation for all feature spaces.}
\label{tab:clustering}
%\end{center}
\end{table}

